Towards Cross-Modality Modeling for Time Series Analytics: A Survey in the LLM Era

The proliferation of edge devices has generated an unprecedented volume of time series data across different domains, motivating various well-customized methods. Recently, Large Language Models (LLMs) have emerged as a new paradigm for time series analytics by leveraging the shared sequential nature of textual data and time series. However, a fundamental cross-modality gap between time series and LLMs exists, as LLMs are pre-trained on textual corpora and are not inherently optimized for time series. Many recent proposals are designed to address this issue. In this survey, we provide an up-to-date overview of LLMs-based cross-modality modeling for time series analytics. We first introduce a taxonomy that classifies existing approaches into four groups based on the type of textual data employed for time series modeling. We then summarize key cross-modality strategies, e.g., alignment and fusion, and discuss their applications across a range of downstream tasks. Furthermore, we conduct experiments on multimodal datasets from different application domains to investigate effective combinations of textual data and cross-modality strategies for enhancing time series analytics. Finally, we suggest several promising directions for future research. This survey is designed for a range of professionals, researchers, and practitioners interested in LLM-based time series modeling.

==> img/taxonomy.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left, font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[!t]
    \centering
    \resizebox{0.87\textwidth}{!}
    {
        \begin{forest}
            forked edges,
            for tree={
                fill=level0!80,
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=9em,font=\normalsize,fill=level1!80,}{},
            where level=2{text width=10em,font=\normalsize,fill=level2!80,}{},
            where level=3{text width=8em,font=\normalsize,fill=level3!60,}{},
            where level=4{text width=10em,font=\normalsize,fill=level4!20,}{},
            where level=5{text width=5em,font=\normalsize,}{},
            [Foundation Models  \\ for Time Series 
                [Standard Time Series
                    [Transformer-based
                        [Pre-trained \\ LLM{,} AM{,} VLM
                            [\textbf{General}: Time-LLM~\cite{jin2023timellm}{,} OFA~\cite{zhou2023one}{,} LLM4TS~\cite{chang2023llm4ts}{,}  PromptCast~\cite{xue2022promptcast}{,} \\   TEMPO~\cite{cao2023tempo}{,} LLMTime~\cite{gruver2023large}{,} Voice2Series~\cite{yang2021voice2series}{,} AutoTimes~\cite{liu2024autotimes}{,} UniTime~\cite{liu2024unitime}, leaf, text width=33em]
                            [\textbf{Finance}: Yu \textit{et al.}~\cite{yu2023temporal}{,} Chen \textit{et al.}~\cite{chen2023chatgpt}{,} Xie \textit{et al.}~\cite{xie2023wall}{,} Wimmer \textit{et al.}~\cite{wimmer2023leveraging}, leaf, text width=33em]
                            [\textbf{Healthcare}: Liu \textit{et al.}~\cite{liu2023large}, leaf, text width=22em]
                        ]
                        [Self-supervised
                            [Generative
                                [\textbf{General:} PatchTST~\cite{nie2022time}{,} Moirai~\cite{woo2024unified}{,} Lag-Llama~\cite{rasul2023lag}{,} \\ TimeSiam~\cite{dong2024timesiam}{,} Timer~\cite{liu2024timer}{,} Das \textit{et al.}~\cite{das2023decoder}{,} UniTS~\cite{gao2024units}{,} \\ TimeGPT-1~\cite{garza2023timegpt}{,} Chronos~\cite{ansari2024chronos}{,} MTSMAE~\cite{tang2022mtsmae},  leaf, text width=24em ]
                            ]
                            [Contrastive
                                [\textbf{General:} TEST~\cite{sun2023test}{,} TimeCLR~\cite{yeh2023toward}, leaf, text width=24em ]
                                [\textbf{Healthcare:} METS~\cite{li2023frozen}, leaf, text width=24em]
                            ]
                            [Hybrid
                                [\textbf{General:} SimMTM~\cite{dong2023simmtm}, leaf, text width=24em ]
                            ]
                        ]
                        [Fully-supervised
                            [\textbf{General}: TimeXer~\cite{wang2024timexer}{,} UniTS~\cite{gao2024units}, leaf, text width=22em]
                        ]
                    ]
                    [non-Transformer-based \\ (MLP RNN CNN)
                        [Self-supervised
                            [Generative
                                [\textbf{General:}  TSMixer~\cite{ekambaram2023tsmixer}, leaf, text width=22em ]
                            ]
                            [Contrastive
                                [\textbf{General:} TF-C~\cite{zhang2022self} {,} TS2Vec~\cite{yue2022ts2vec} {,}  CLUDA~\cite{ozyurt2022contrastive} , leaf, text width=22em ]
                            ]
                        ]
                        [Fully-supervised
                            [\textbf{General}: TTMs~\cite{ekambaram2024ttms}{,} TimesNet~\cite{wu2022timesnet}{,} RWKV-TS~\cite{hou2024rwkv}, leaf, text width=25em]
                        ]
                    ]
                    [Diffusion-based
                        [\textbf{General:} TimeGrad~\cite{rasul2021autoregressive} {,} D$^3$VAE~\cite{li2022generative} {,}  TransFusion~\cite{sikder2023transfusion} {,}  ScoreGrad~\cite{yan2021scoregrad} {,} \\  Biloš \textit{et al.}~\cite{bilovs2022modeling} {,}  Crabbé \textit{et al.}~\cite{crabbe2024time} {,}  TimeDiff~\cite{shen2023non} {,}  Wang \textit{et al.} ~\cite{wang2023observed} {,}   DiffTime~\cite{coletta2024constrained}, leaf, text width=35em ]
                        [\textbf{Finance:} {FTS-Diffusion}~\cite{huang2024generative}, leaf, text width=31.7em ]
                        [\textbf{Power:} {DiffLoad}~\cite{wang2023diffload}, leaf, text width=31.7em ]
                        % [\textbf{Application:}, leaf, text width=22em ]
                    ]
                ]
                [Spatial Time Series
                    [Transformer-based
                        [Pre-trained LLM
                            [\textbf{Transportation:} ST-LLM~\cite{liu2024spatial}{,} TPLLM~\cite{ren2024tpllm}, leaf, text width=22em ]
                            [\textbf{General:} GATGPT~\cite{chen2023gatgpt}, leaf, text width=22em ]
                        ]
                        [Self-supervised
                            [Generative
                                [\textbf{Transportation:} STEP~\cite{shao2022pre}, leaf, text width=22em]
                                [\textbf{Climate:} W-MAE~\cite{man2023w}{,} MetePFL~\cite{chen2023prompt}{,}  FengWu~\cite{chen2023fengwu}, leaf, text width=22em ]
                                [\textbf{General:} UniST~\cite{yuan2024unist}, leaf, text width=22em]
                            ]
                        ]
                        [Fully-supervised
                            [\textbf{Transportation:} CPPBTR~\cite{duan2019pre} {,} TFM~\cite{wang2023building}, leaf, text width=22em ]
                            [\textbf{Climate:} FourCastNet~\cite{pathak2022fourcastnet} {,} FedWing~\cite{chen2023spatial} {,} Pangu-Weather~\cite{bi2023accurate}{,} ClimaX~\cite{nguyen2023climax}, leaf, text width=33em ]
                        ]
                    ]
                    [non-Transformer-based \\ (MLP RNN CNN)
                        [Self-supervised
                            [\textbf{General:} SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                    ]
                    [Diffusion-based
                        [\textbf{General:} {DiffSTG}~\cite{wen2023diffstg} {,} {DSTPP}~\cite{yuan2023spatio} {,} {DYffusion}~\cite{cachay2023dyffusion} {,} {Yun \textit{et al.}}~\cite{yun2023imputation} {,} {USTD}~\cite{hu2023unifying} {,} {PriSTI}~\cite{liu2023pristi}, leaf, text width=42em ]
                    ]
                ]
                [Others
                    [Transformer-based
                        [Pre-trained LLM
                            [\textbf{Mobility:} {AuxMobLCast}~\cite{xue2022leveraging} {,} {LLM-Mob}~\cite{wang2023i}, leaf, text width=22em ]
                            [\textbf{Event:} {LAMP}~\cite{shi2023language} {,} {Gunjal \& Durrett \textit{et al.}}~\cite{gunjal2023drafting}, leaf, text width=22em ]
                        ]
                        [Self-supervised
                            [Generative
                                [\textbf{Mobility:} {GTM}~\cite{lin2024gtm}, leaf, text width=22em]
                                [\textbf{Event:} {NYUTron}~\cite{jiang2023health} {,} {GatorTron}~\cite{yang2022large}, leaf, text width=22em ]
                            ]
                            [ Contrastive  % {TrajCL}~\cite{chang2023contrastive},
                                 [\textbf{Mobility:} {TrajCL}~\cite{chang2023contrastive}, leaf, text width=22em]
                            ]
                        ]
                    ]
                    [non-Transformer-based \\ (MLP RNN CNN)
                        [Self-supervised
                            [Generative
                               [\textbf{Mobility:} {Trembr}~\cite{fu2020trembr}, leaf, text width=22em ]
                            ]
                            [Contrastive
                               [\textbf{Mobility:} {MMTEC}~\cite{lin2023pretraining}, leaf, text width=22em ] 
                            ]
                            [Hybrid
                               [\textbf{Mobility:} {START}~\cite{jiang2022self}, leaf, text width=22em ] 
                            ]
                        ]
                    ]
                    [Diffusion-based
                        [\textbf{Mobility:} {TrajGDM}~\cite{chu2024simulating} {,} {DiffTraj}~\cite{zhu2024difftraj}, leaf, text width=22em ]
                    ]
                ]
            ]
        \end{forest}
    }    
\caption{A comprehensive taxonomy of TSFMs, categorized according to data and methodologies.}
\label{fig:taxonomy}
\end{figure*}
% , categorized according to methodologies (i.e., unconditioned vs. conditioned), tasks (e.g., predictive versus generative), and applications.
% Single-Modality
%  [xxx, leaf, text width=22em ]

% others： 展开
% 
                
